Truly Subcubic Min-Plus Product for Less Structured Matrices, with Applications

The goal of this paper is to get truly subcubic algorithms for Min-Plus product for less structured inputs than what was previously known, and to apply them to versions of All-Pairs Shortest Paths (APSP) and other problems. The results are as follows: (1) Our main result is the first truly subcubic algorithm for the Min-Plus product of two $n\times n$ matrices $A$ and $B$ with $\text{polylog}(n)$ bit integer entries, where $B$ has a partitioning into $n^{\epsilon}\times n^{\epsilon}$ blocks (for any $\epsilon>0$) where each block is at most $n^\delta$-far (for $\delta<3-\omega$, where $2\leq \omega<2.373$) in $\ell_\infty$ norm from a constant rank integer matrix. This result presents the most general case to date of Min-Plus product that is solvable in truly subcubic time. (2) The first application of our main result is a truly subcubic algorithm for APSP in a new type of geometric graph. Our result extends the result of Chan'10 in the case of integer edge weights by allowing the weights to differ from a function of the end-point identities by at most $n^\delta$ for small $\delta$. (3) In the second application we consider a batch version of the range mode problem in which one is given a length $n$ sequence and $n$ contiguous subsequences, and one is asked to compute the range mode of each subsequence. We give the first $O(n^{1.5-\epsilon})$ time for $\epsilon>0$ algorithm for this batch range mode problem. (4) Our final application is to the Maximum Subarray problem: given an $n\times n$ integer matrix, find the contiguous subarray of maximum entry sum. We show that Maximum Subarray can be solved in truly subcubic, $O(n^{3-\epsilon})$ (for $\epsilon>0$) time, as long as the entries are no larger than $O(n^{0.62})$ in absolute value. We also improve all the known conditional hardness results for the $d$-dimensional variant of Maximum Subarray.

==> intro-old.tex <==
% - maximum subarray+history
% - kadane's algorithm and improvements
% - conditional lower bounds
% - issues: (1) they are not tight for d>3, (2) what if the entries in the arrays are bounded? can we get a faster algorithm? could be useful in practice? in the 2d reduction to distance product, the weights blow up, so the known distance product algorithm doesn't immediately apply. However, the known reduction does give structured matrices:
% Bounded Monge matrices.
% Is distance product faster than cubic for such matrices?
% Relatedly, Bounded Differences Matrices were shown to have a faster algorithm. Every bounded difference matrix is a Bounded Monge matrix (even if it is only rowwise or columnwise), so any algorithm for bounded Monge matrices would also imply the result for bounded diff matrices. also, bounded monge are not bounded difference at all: 100, -50 | 50, 0. Completely unclear how to modify bdd algorithm for the bounded Monge case.
% a truly subcubic algorithm would largely increase our knowledge in apsp

% contributions:
% (1) tight conditional lower bounds for all d
% (2) high conditional lower bounds for all d and bounded weights
% (3) truly subcubic algorithm for small weights.

In the Maximum Subarray problem, one is given a real valued square matrix and is asked to find the contiguous submatrix of maximum entry sum. First studied by Bentley~\cite{bentley84alg}, the problem has many applications, for instance in graphics (see \cite{tamaki1998algorithms}) and in databases \cite{databases-app1,databases-app2,databases-app2j,databases-app3,databases-app4}.

The Maximum Subarray problem can be generalized to arbitrary $d$ dimensions: here one is given a $d$-dimensional grid (or tensor) with $n$ coordinates in each dimension (i.e. $[n]^d$), each point in the grid has a real value, and one is asked to return the contiguous subgrid of maximum entry sum.
In 1D, Kadane's algorithm (presented in \cite{bentley84alg}) achieves a linear, $O(n)$ running time. Bentley~\cite{bentley84} showed how to use Kadane's algorithm to solve the $2$D variant of the Maximum Subarray problem in $O(n^3)$ time; the same approach gives an $O(n^{2d-1})$ time algorithm, ``Kadane's algorithm'', for the $d$ dimensional version for all $d$. Tamaki et al.~\cite{tamaki1998algorithms} and Takaoka~\cite{Takaoka02} showed how to use divide-and-conquer to efficiently reduce the $2$D Maximum Subarray problem on an $n\times n$ matrix to the $(\min, +)$-product of two $n\times n$ matrices (a problem equivalent to All-Pairs Shortest Paths (APSP) in $n$ node graphs). Using the fastest APSP algorithm to date by Williams~\cite{williams2014faster}, one obtains the fastest 2D Maximum Subarray algorithm to date, running in $n^3/2^{\Theta(\sqrt{\log n})}$ time. This algorithm can be used to give the fastest known running time  $n^{2d-1}/2^{\Theta(\sqrt{\log n})}$ for the $d$-dimensional version of the problem as well.

In recent years, fine-grained complexity has yielded conditional lower bounds for Maximum Subarray. Backurs et al.~\cite{backurs2016tight} and Vassilevska W. and Williams~\cite{vw10j} showed that an $O(n^{3-\eps})$ time algorithm for $2$D Maximum Subarray for $\eps>0$ would imply an $O(n^{3-\eps'})$ time algorithm for $(\min,+)$-product (and hence APSP), for $\eps'$. Together with the reductions of \cite{tamaki1998algorithms,Takaoka02}, this implies that the $2$D Maximum Subarray problem is subcubically equivalent to APSP. One of the main hardness hypotheses of fine-grained complexity is that APSP requires $n^{3-o(1)}$ time (in the word RAM model with $O(\log n)$ bit words). Under this hypothesis, the best known algorithms for $2$D Maximum Subarray are essentially optimal, up to $n^{o(1)}$ factors.

While the fastest known algorithm for $d$-Dimensional Maximum Subarray runs in $n^{2d-1-o(1)}$ time, the known conditional lower bound~\cite{backurs2016tight} is much lower for $d>2$, $n^{ 3d/2-o(1)}$. A natural question is thus, is there a faster algorithm for $d>2$, or can the conditional lower bounds be improved?

Another intriguing question is whether the $2$D Maximum Subarray problem can be solved in truly subcubic, $O(n^{3-\eps})$ time for $\eps>0$ when the entries of the input matrix are integers, small in absolute value. Such an algorithm would be very interesting in practice, as the matrix values often represent such small discrete values.
%say in the interval $\{-M,\ldots,M\}$ where $M$ is small?
As a motivation for why a faster algorithm might exist in this case, note that the $(\min,+)$-product of $n\times n$ matrices with entries in $\{-M,\ldots,M\}\cup \{\infty\}$ has an algorithm running in $\tilde{O}(Mn^\omega)$ time \cite{AlonGM97} where $\omega<2.373$ is the exponent of square matrix multiplication \cite{cw90,stothers,vmmult,legallmult}. That is, for small enough $M$, the $(\min,+)$-product problem has a truly subcubic time algorithm.
Due to the equivalence between $(\min,+)$-product and Maximum Subarray, it stands to reason that such an algorithm might exist for the small entry Maximum Subarray problem as well. Unfortunately, the known reductions from Maximum Subarray to $(\min,+)$-product blow up the matrix entries, so that even if the maximum subarray entries are in $\{-1,0,1\}$, the resulting matrices whose $(\min,+)$-product we want to compute might have entries that are quadratic in $n$. Thus, one cannot simply use the known faster algorithms for small entry $(\min,+)$-product to speed-up the Maximum Subarray problem with small entries.  On the lower bound end, there doesn't seem to be a way to take an instance of $(\min,+)$-product with arbitrarily large entries and to create a maximum subarray instance with small entries. Thus, there is no obvious way to show that the small entry case is hard.


\subsection{Our results.}
We present two sets of results. The first is a truly subcubic algorithm for $2$D Maximum Subarray with bounded entries, which is obtained as a corollary to a new powerful $(\min,+)$-product algorithm which is truly subcubic for a large class of inputs, subsuming and generalizing all known classes of inputs for which truly subcubic algorithms were known. Our second result is a set of conditional lower bounds for Maximum Subarray in $d$ dimensions, showing in particular that the $\tilde{O}(n^{2d-1})$ time algorithms are essentially tight.

\paragraph{Min-Plus product for bounded discrete derivative matrices and faster $2$D Maximum Subarray with small entries.}

Examining
% Nevertheless, there is some structure that one can potentially exploit, algorithmically. If one runs
Tamaki et al. and Takaoka's reduction of Maximum Subarray to $(\min,+)$-product, it can be seen that starting with a maximum subarray instance with entries in $\{-M,\ldots,M\}$,
one obtains $n\times n$ matrices $A$ and $B$ with the following {\em bounded discrete derivative} (BDD) structure:
\[\forall X\in \{A,B\},\forall i,j\in [n-1],~|X[i,j]+X[i+1,j+1]-X[i,j+1]-X[i+1,j]|\leq M.\]
The question becomes, can one perform the $(\min,+)$-product of BDD matrices in truly subcubic time, when $M$ is small? This question is of independent interest.

There are several known results on faster $(\min,+)$-product for structured matrices. We already mentioned one- when the matrices have small integer entries. A related property is when each row of one of the matrices has a small number of distinct values \cite{Yuster09}. Arguably the most general result so far is by Bringmann et al.~\cite{BringmannGSW16} who showed that a truly subcubic algorithm for $(\min,+)$ product exists if one of the matrices has ``bounded differences" in each row (or in each column), that is, if  $\forall i,j~|A[i,j]-A[i,j+1]|\leq M$ for small $M$. In fact, the algorithm runtime is truly subcubic for any $M\leq O((n^{3-\omega-\eps})$ for some $\eps>0$. 

% for small $M$. more precisely, for all $M\leq O(n^{3-\omega-\eps})$, the algorithm runs in  $\tilde{O}(n^{3-\Omega(\eps)})$ time.

It is not hard to see that if $A$ has bounded differences in its rows (or columns), then it is also BDD. Moreover, there exist many matrices that are BDD but do not have bounded differences or bounded entries. Thus a truly subcubic time $(\min,+)$-product algorithm that works when one of the matrices is BDD and the other is arbitrary, would subsume and significantly extend the known cases for which fast $(\min,+)$-product algorithms are known to exist. (For the Maximum Subarray application it would of course suffice to only handle the case when both matrices are BDD.)

Our first result is:
\begin{theorem}\label{thm:any_with_BDD}
There exists an $\tilde{O}(M^{1/6}n^{(15+\omega)/6})$ time algorithm that computes the $(\min,+)$-product of two $n \times n$ matrices $A$ and $B$, where $A$ is an arbitrary integer matrix, and $B$ has $M$-bounded discrete derivatives. When $M=O(1)$ and $\omega \le 2.373$, the algorithm has run time $O(n^{2.8955})$.
\end{theorem}

As an immediate corollary, we obtain an $\tilde{O}(M^{1/6}n^{(15+\omega)/6})$ time algorithm that solves the Maximum Subarray problem in $2$D for $n\times n$ matrices with entries in $\{-M,\ldots,M\}$.

Along the way to our result above, we slightly improve the known algorithms for $(\min,+)$-product of matrices with bounded entries. It is known (see e.g. \cite{Yuster09}, Lemma 3.3) that the $(\min,+)$-product of $n\times n$ matrices $A$ and $B$ where $B$ is arbitrary and $A$ has entries in $\{-M,\ldots, M\}\cup\{\infty\}$, can be computed in time $\tilde{O}(Mn^{(3+\omega)/2})$ (and slightly faster with rectangular matrix multiplication). We improve the dependence on $M$. 

\begin{theorem}\label{thm:small_weight_times_large_weight}
The $(\min,+)$-product of two $n\times n$ integer matrices $A$ and $B$, where $A$ has entries in $\{-M,\ldots, M\}\cup\{\infty\}$ and $B$ is arbitrary can be computed in $\tilde{O}(\sqrt{M}n^{(3+\omega)/2})$ time.
\end{theorem}


\paragraph{Conditional lower bounds for $d$-Dimensional Maximum Subarray.}
Backurs et al.~\cite{backurs2016tight} showed that the $d$-Dimensional Maximum Subarray problem requires $n^{3d/2-o(1)}$ time (in the word-RAM model of computation) under the following popular hardness assumption (see e.g. \cite{vsurvey}):

\begin{hypothesis}[Max-Weight $k$-Clique Hypothesis]
In the word-RAM model with $O(\log n)$ bit words, there is no $O(n^{k-\eps})$ time algorithm for $\eps>0$ that can find a $k$-Clique of maximum weight in a given $n$-node graph with edge weights in $\{-n^{ck},\ldots,n^{ck}\}$ for large enough constant $c$.\end{hypothesis}  

Our first hardness result is an improvement of the lower bound of Backurs et al., showing that Kadane's algorithm for $d$-Dimensional Maximum Subarray is conditionally tight:

\begin{theorem}\label{thm:subarray_lowerbound}
Under the Max-Weight $k$-Clique Hypothesis, in the word-RAM model with $O(\log n)$ bit words, the $d$-Dimensional Maximum Subarray problem requires $n^{2d-1-o(1)}$ time.
\end{theorem}

We were able to show that the $2$D Maximum Subarray problem can be solved faster when the matrix entries are bounded. One might wonder whether such an improvement is possible for $d>2$ as well? The simple reduction from $d$-Dimensional Maximum Subarray to $2$-Dimensional Maximum Subarray, unfortunately blows up the entries, and one cannot use the subcubic algorithm that we developed in a straightforward way. While an improvement is still possible for larger $d$, we show under a popular hardness assumption that at best one would be able to save a factor of $n^{1+o(1)}$ over the runtime of Kadane's algorithm.

The hardness assumption we use is the $\ell$-Uniform Hyperclique assumption used in prior work (see e.g. \cite{LincolnWW18,AbboudBDN18}):

\begin{hypothesis}[$\ell$-Uniform $k$-Hyperclique Hypothesis]
Let $k>\ell\geq 3$ be integers.
In the word-RAM model with $O(\log n)$ bit words, there is no $O(n^{k-\eps})$ time algorithm for $\eps>0$ that can find a hyperclique on $k$ nodes in a given $n$-node $\ell$-uniform hypergraph.\end{hypothesis}  

The hypothesis is very believable for a variety of reasons. It is known (see \cite{LincolnWW18}) that the natural extension of the techniques used to solve $k$-clique (in graphs) will not solve $k$-hyperclique in $\ell$-uniform hypergraphs faster than $n^k$. Moreover, there are known
reductions from notoriously difficult problems such as Exact
Weight $k$-Clique (a problem harder than Max Weight $k$-Clique) \cite{AbboudBDN18}, Max $\ell$-SAT and even harder Constrained
Satisfaction  Problems  (CSPs) \cite{Williams05,LincolnWW18}  to $k$-hyperclique in $\ell$-uniform hypergraphs so  that
if  the  hypothesis  is  false,  then  all  of  these  problems  have surprisingly improved algorithms. 

We prove:
\begin{theorem}\label{thm:bounded_subarray_lowerbound}
Fix any $d\geq 3$.
Under the $3$-Uniform $(2d-2)$-Hyperclique Hypothesis, in the word-RAM model with $O(\log n)$ bit words, the $d$-Dimensional Maximum Subarray problem on matrices with entries in $\{-2^{O(d)},\ldots,2^{O(d)}\}$ requires $n^{2d-2-o(1)}$ time.
\end{theorem}
That is, for any constant $d$, solving the problem in matrices with entries bounded by a constant is $n^{2d-2-o(1)}$-hard.


% The most general structural property known so far, for which truly subcubic algorithms are known is the so called bounded difference property, in which adjacent entries of the matrices must be close to each other. The 

